Near- And Mid-Infrared Imaging Study of Young Stellar Objects around LkH$\alpha$ 234

We present high-resolution ($0\farcs2$) near-infrared images of the area surrounding the Herbig Be star LkH$\alpha$ 234 taken with the Coronagraphic Imager with Adaptive Optics (CIAO) and the adaptive optics on the Subaru Telescope. The near-infrared ($J$, $H$, $K$, $L'$ and $M'$ bands) images reveal circumstellar structures around LkH$\alpha$ 234 in detail. Eight young stellar object (YSO) candidates (Object B, C, D, E, F, G, NW1, and NW2) were detected at 2$\arcsec$--11$\arcsec$ from LkH$\alpha$ 234. Objects B and C are likely variable stars, which is consistent with a young evolutionary status. Three objects (LkH$\alpha$ 234, NW1, and NW2) were identified in the 11.8 $\micron$ (SiC) and 17.65 $\micron$ images obtained with the Long Wavelength Spectrometer (LWS) on the Keck Telescope. NW1 and NW2 are thought to be embedded young stars. We suggest that NW1 and not LkH$\alpha$ 234 is the source illuminating the reflection nebula west of LkH$\alpha$ 234, although Object G may be another candidate. In our images, these objects are located at the center of the 2 $\micron$ polarization, and NW1 resides at the center of a monopolar cavity. The SED of NW1 suggests that it is a YSO with a spectral type of B6--7. Object F and G were discovered by our observations at $1\farcs9$ and $2\farcs3$, respectively, from LkH$\alpha$ 234, and their proximity to LkH$\alpha$ 234 suggests that they may be its lower-mass companions.

==> 00README.tex <==
nohypertex
